Survey of Gravitationally Lensed Objects in HSC Imaging (SuGOHI). IX. Discovery of Strongly Lensed Quasar Candidates

We report the discovery of new lensed quasar candidates in the imaging data of the Hyper Suprime-Cam Subaru Strategic Program (HSC-SSP) DR4, covering $1\,310~{\rm deg}^2$ of the sky with seeing of $\approx0.6''$. In addition to two catalogs of MILLIQUAS and AllWISEAGN, which contain confirmed and candidate quasars, we preselect quasar sources using color cuts from the HSC ($grizy$) and unWISE ($W1+W2$) photometric data based on SDSS spectroscopic catalogs. We search for the presence of multiple point sources with similar color through the convolution of the Laplacian of the preselected quasar image cutouts with the Laplacian of the point spread function, resulting in a reduction of lens candidates from $1\,652\,329$ to $121\,511$ ($7.4\%$). After visual binary classification, we grade $6\,199$ ($0.4\%$) potential lenses on a scale of 0 to 3, with 3 indicating a lens and 0 indicating a non-lens. Finally we obtain 162 lens candidates with an average grade of $\geq2$, and among them, we successfully recover 18 known lenses. By fitting the light distribution and removing the known contaminants, we discover that 57 new systems contain at least two point sources and a galaxy in between, including 10 possible quadruply lensed quasars. This new sample of lens candidates exhibits a median separation of $1.26''$ and a magnitude limit of $i\approx22$. Spectroscopic or high-resolution imaging follow up on these newly discovered lensed quasar candidates will further allow their natures to be confirmed.

==> tabs/numbers_old.tex <==
\begin{tabular}{crrrrrrr}
\hline\hline
\multicolumn{1}{c}{Catalog} & \multicolumn{1}{c}{Input} & \multicolumn{1}{c}{Algorithm} & \multicolumn{1}{c}{[\%]}& \multicolumn{1}{c}{Phase 1} & \multicolumn{1}{c}{[\%]}& \multicolumn{1}{c}{$G_{\rm av}\geq2$} & \multicolumn{1}{c}{[\%]}\\
\hline
          HSC+unWISE &    1587892 &     233270 &      14.69 &       6111 &       0.38 &        162 &      0.010 \\
           MILLIQUAS &     150316 &       4129 &       2.75 &        376 &       0.25 &         38 &      0.025 \\
          AllWISEAGN &      49943 &       1490 &       2.98 &        117 &       0.23 &         22 &      0.044 \\
\hline
               Total &    1652329 &     234424 &      14.19 &       6199 &       0.38 &        162 &      0.010 \\
\hline
\end{tabular}

